Differentiable Causal Discovery Under Latent Interventions

Recent work has shown promising results in causal discovery by leveraging interventional data with gradient-based methods, even when the intervened variables are unknown. However, previous work assumes that the correspondence between samples and interventions is known, which is often unrealistic. We envision a scenario with an extensive dataset sampled from multiple intervention distributions and one observation distribution, but where we do not know which distribution originated each sample and how the intervention affected the system, \textit{i.e.}, interventions are entirely latent. We propose a method based on neural networks and variational inference that addresses this scenario by framing it as learning a shared causal graph among an infinite mixture (under a Dirichlet process prior) of intervention structural causal models. Experiments with synthetic and real data show that our approach and its semi-supervised variant are able to discover causal relations in this challenging scenario.

==> cm-paper/table_experiments.tex <==

\begin{table}
\small
    \centering
    \begin{tabular}{lcccccc}
    \toprule
        \textbf{Model Type} &  $e$  & \textbf{latent} & \textbf{unknown} & \textbf{known} & \textbf{observational} \\
    \midrule
        &&\multicolumn{3}{c}{\textit{Stochastic Interventions:}}&&\\
        Linear Gaussian  &     & $5.9\pm 6.2$ & $3.4\pm3.2$   & $ 0.5\pm1.3 $& $10.3\pm7.8$\\
        Non-Linear Gaussian & 1 &   $12.2\pm3.9$ & $10.3\pm2.5$ & $7.0\pm3.6$ & $13.7\pm3.8$ \\
        Non-Linear Non-Gaussian &  &   $8.7\pm6.6$  & $8.0\pm2.7$ & $6.6\pm2.2$ & $11.3\pm5.0$ \\
    \midrule
        Linear Gaussian &  &   $27.2 \pm 6.2$ & $24.1 \pm 5.8$ & $15.6 \pm 6.0$& $39.6 \pm 5.0$ \\
        Non-Linear Gaussian & 4  &   $35.8\pm3.8$ & $30.3\pm5.3$ & $27.7\pm4.3$ & $37.5\pm5.2$ \\
        Non-Linear Non-Gaussian &   & $36.1 \pm 4.4$ & $35.5 \pm 8.1$& $31.5 \pm 5.6$&  $40.2\pm6.9$\\
    \midrule
        &&\multicolumn{3}{c}{\textit{Imperfect Interventions:}}&&\\
        Linear Gaussian &    & $ 5.8 \pm 4.2 $ & $6.2 \pm 3.06  $ & $ 4.7 \pm 3.6 $ & $ 10.4 \pm 2.9 $\\
        Non-Linear Gaussian &  1 &  $ 9.3 \pm 2.4 $ & $ 8.9 \pm 2.5 $ & $ 7.8 \pm 3.9  $ & $ 10.5 \pm 2.8 $ \\
        Non-Linear Non-Gaussian &  &   $ 8.8 \pm 3.0 $  & $ 9.1 \pm 3.5 $ & $ 7.9 \pm 1.4$ & $11.5\pm5.4$\\
    \midrule
        Linear Gaussian &  &  $35.9\pm 8.3$ & $29.7 \pm 5.6$ & $17.7\pm7.9$ & $39.1 \pm 9.1$ \\
        Non-Linear Gaussian & 4  &  $ 32.1 \pm 6.0 $ & $32.6\pm5.8$& $ 32.8\pm 5.4 $ & $39.8 \pm 9.3$ \\
        Non-Linear Non-Gaussian & &  $ 30.4 \pm 12.2$ &  $ 30.2 \pm 11.2 $ & $25.8 \pm 3.9$ & $36.7 \pm 9.8$ \\
    \bottomrule
    \end{tabular}
    \caption{Hamming distances on synthetic 10 variable SCMs.}
    \label{tab:perfectdagsingle}
\end{table}

